NYTWIT: A Dataset of Novel Words in the New York Times

We present the New York Times Word Innovation Types dataset, or NYTWIT, a collection of over 2,500 novel English words published in the New York Times between November 2017 and March 2019, manually annotated for their class of novelty (such as lexical derivation, dialectal variation, blending, or compounding). We present baseline results for both uncontextual and contextual prediction of novelty class, showing that there is room for improvement even for state-of-the-art NLP systems. We hope this resource will prove useful for linguists and NLP practitioners by providing a real-world environment of novel word appearance.

==> tab_examples.tex <==
\begin{table*}
    \centering
    \small
    \begin{tabular}{lllll}
        \toprule
        Time & URL & Word & Type & Comments \\
         \midrule
        02-08-2018 11:01:12 & [url] & blotchier & inflection &  \\
        10-16-2018 23:57:39 & [url] & paleoproteomics & domain &  \\
        03-23-2018 15:03:35 & [url] & vacuuuuuuuuum & lengthening &  \\
        05-21-2018 11:02:32  & [url] & smellwalks & compound &  \\
        05-02-2018 15:02:27 & [url] & chipster & blend & `chip' + `hipster' \\
        \bottomrule
    \end{tabular}
    \caption{Data examples. \todo{do we share actual urls here?}}
    \label{tab:examples}
\end{table*}

